Family Ties: Relating Poncelet 3-Periodics by their Properties

We compare loci types and invariants across Poncelet families interscribed in three distinct concentric Ellipse pairs: (i) ellipse-incircle, (ii) circumcircle-inellipse, and (iii) homothetic. Their metric properties are mostly identical to those of 3 well-studied families: elliptic billiard (confocal pair), Chapple's poristic triangles, and the Brocard porism. We therefore organized them in three related groups.

==> _not_used/130_app_equilaterals.tex <==
Referring to Figure~\ref{fig:isodynamic-equis}, the pedal (resp. antipedal) triangles of the isodynamic points $X_{15}$ and $X_{16}$ (resp. isogonic points $X_{13}$ and $X_{14}$) are equilaterals centered on $X_{396}$ and $X_{395}$ (resp.  $X_{5463}$ and $X_{5464}$) \cite{etc}.

Let $A$ denote the area of a triangle and $A_k$, $k={13,14,15,16}$ denote the area of said equilaterals. Peter Moses has kindly contributed the following expressions \cite{moses2020-private-equilaterals}:

\begin{align*}
A_{13}/A =& 2 + \frac{2 \cot\omega}{\sqrt{3}},\;\;\;A_{14}/A = 2 - \frac{2 \cot\omega}{\sqrt{3}}\\
A_{15}/A =& \frac{-3 + \sqrt{3} \cot\omega}{2(\csc^2\omega - 4)},\;\;\;
A_{16}/A = \frac{-3 - \sqrt{3} \cot\omega}{2(\csc^2\omega - 4)}
\end{align*}

\begin{corollary}
For any triangle:
\[ \frac{A_{13}}{A_{14}}=\frac{A_{16}}{A_{15}}= \frac{\cot\omega+\sqrt{3}}{\Sha -\sqrt{3}} \]
\end{corollary}

\begin{corollary}
The Brocard porism conserves $A_{13}/A_{14}$ and $A_{16}/A_{15}$.
\end{corollary}

%\[
%\frac{A_{16}}{A_{15}}= {\frac { \left( s_1^{2}+s_2^{2}+s_3^{2} \right)  \left( s_1^{2}+s_2^{2}+s_3^{2}+2\,2\sqrt {3}A \right) }{2\,s_1^{4}-2\,s_1^{2}s_2^{2}-2\,s_1^{2}s_3^{2}+2\,s_2^{4}-2\,s_2^{2}s_3^{2}+2\,s_3^{4}}}-1\]

%Using Conwayng the above over the Brocard porism vertices (Proposition~\ref{prop:orbita}) and using a CAS for simplication obtain:

%\[\frac{A_{16}}{A_{15}}= \frac{(\sqrt{3}h-3d)^2}{(\sqrt{3}h+3d)^2}\]

%A further simplification using Lemma \ref{lem:7} leads to the result.
%\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/0130_broc_isos.eps}
    \caption{The pedal (resp. antipedal) triangles (orange, resp. purple) of the isodynamic points $X_{15}$ and $X_{16}$ (resp. isogonic points $X_{13}$ and $X_{14}$) are equilaterals centered on $X_{396}$ and $X_{395}$, collinear with $X_6$ (resp. $X_{5463}$ and $X_{5464}$, collinear with $X_3$) \cite{etc}. Over the porism, the area ratios $A_{16}/A_{15}$ and $A_{13}/A_{14}$ are invariant and identical. The loci of $X_{396}$ and $X_{395}$ are circles (dashed orange) as are those of $X_{5463}$ and $X_{5464}$ (not shown).
    \href{https://youtu.be/s4DF-iZZO8Y}{Video}}
    \label{fig:isodynamic-equis}
\end{figure}

The centroid of the pedal triangle of $X_{15}$ (resp. $X_{16}$) is  $X_{396}$ (resp. $X_{395}$).

\begin{proposition}
The locus of $X_{15}$ and $X_{16}$ pedal centroids $X_{396}$ and $X_{395}$ are the following circles:

\[C_{395}= \left[ 0,  \frac {R \left(  3(\Sha^2+1)-2\,\sqrt {3}\;\Sha \right) 
 \left( \Sha+ \sqrt {3} \right) }{3\sqrt { \Sha^2-3} \left(  
\Sha^2+1 \right) }
 \right],\;\;
r_{395}=\frac{R (\sqrt{3}\Sha +3)}{3(\Sha^2+1)}\]
\[C_{396}= \left[ 0,  \frac {R \left(3\, ( \Sha^2+1 )+ 2\,\sqrt {3}\;\Sha \right) 
 \left(  \Sha -\sqrt {3}\right) }{3\sqrt {\Sha^2-3} \left( \Sha^{2}+1 \right) }
 \right],\;\;
r_{396}=\frac{R (\sqrt{3}\Sha -3)}{3(\Sha^2+1)}\]

\end{proposition}

\begin{proof}
Obtained via CAS.
\end{proof}

\begin{remark}
Notice the ratio $r_{395}/r_{396}$ is equal to $A_{396}/A_{395}$.
\end{remark}

\begin{proposition}
The locus of $X_{13}$ and $X_{14}$ antipedal centroids $X_{5463}$ and $X_{5464}$ are the following circles:
\end{proposition}

\subsection{Homothetic Pair}

In \cite{reznik2020-similarityII} we studied invariants both in the Brocard porism and the {\em homothetic} family, i.e., Poncelet 3-periodics inscribed in an outer ellipse with semi-axes $(a,b)$ and circumscribed about an axis-aligned concentric one with semi-axes $(a/2,b/2)$. We showed that like the Brocard porism, the homothetic pair is also {\em equibrocardal}, i.e., it conserved $\omega$. Furthermore, the area of its triangles is constant. However its Brocard points are not stationary (in fact their loci are two angled ellipses similar to the pair \cite{garcia2020-brocard}.

The claims below refer to properties over the homotheric family. Referring to Figure~\ref{fig:homot-equis}:

\begin{corollary}
$A_k$, $k=13,14,15,16$ are all invariant and given by:
\textcolor{red}{ronaldo}
\end{corollary}

This stems from the fact that these four areas only depend, for a generic triangle, on $\omega$ and the area of the triangle, both constant in the homothetic family.

\begin{proposition}
The locus of $X_k$, $k=13,14,15,16$ are the following circles:
\textcolor{red}{ronaldo}
\end{proposition}

\begin{proposition}
The locus of center $X_{5463}$ (resp. $X_{5464}$) of the first (resp. second) isogonic antipedal, coincides with the circular locus of $X_{13}$ (resp. $X_{14}$). 
\end{proposition}

\begin{proposition}
The locus of the centers $X_{396}$ (resp. $X_{395}$) of the isodynamic equilateral pedals are two ellipses given by:
\textcolor{red}{ronaldo}
\end{proposition}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/0140_homot_isos.eps}
    \caption{The homothetic Poncelet family (stationary $X_2$) is equibrocardal (conserves $\omega$) and its triangles (blue) have invariant area. The loci of $X_k,k=13,14,15,16$ are circles concentric with the ellipses \href{https://youtu.be/ZwTfwaJJitE}{Video}. Since areas $A_{15}$, $A_{16}$, $A_{13}$, $A_{14}$ only depend on $\omega$, they are individually invariant. The loci of $X_{396}$ and $X_{395}$ are ellipses whereas those of $X_{5463}$ and $X_{5464}$ are circles.
    \href{https://youtu.be/7qoxAaG8sbk}{Video}}
    \label{fig:homot-equis}
\end{figure}
